Search for resonances in the mass distribution of jet pairs with one or two jets identified as $b$-jets in proton-proton collisions at $\sqrt{s}=13$ TeV with the ATLAS detector

A search for new resonances decaying into jets containing b-hadrons in $pp$ collisions with the ATLAS detector at the LHC is presented in the dijet mass range from 0.57 TeV to 7 TeV. The dataset corresponds to an integrated luminosity of up to 36.1 fb$^{-1}$ collected in 2015 and 2016 at $\sqrt{s} = 13$ TeV. No evidence of a significant excess of events above the smooth background shape is found. Upper cross-section limits and lower limits on the corresponding signal mass parameters for several types of signal hypotheses are provided at 95% CL. In addition, 95% CL upper limits are set on the cross-sections for new processes that would produce Gaussian-shaped signals in the di-b-jet mass distributions.

==> section_auxmat.tex <==
\begin{figure}[!ht]
\begin{center}
\includegraphics[scale=0.5, angle=0]{figure/FinalPlots/mass_data_mc_ratio_fin.pdf}
\end{center}
\caption{The mass distributions for the inclusive one $b$-tagged (dot) selection and two $b$-tagged (square) selection using an integrated luminosity of $36.1$ \ifb. The inclusive one $b$-tagged Pythia8 MC distribution (blue line) is normalized to the inclusive one $b$-tagged data. The two $b$-tagged Pythia8 MC distribution (blue dashed line) is normalized to the two $b$-tagged data. Ratios between data and MC are also shown. The systematic uncertainty band is dominated by the $b$-tagging scale factor and the $b$-jet energy scale.}
\label{fig:25mass_scale}
\end{figure}

% \begin{figure}[!ht]
% \begin{center}
% \subfigure[High mass region]{
% \includegraphics[scale=0.4, angle=0]{figure/FinalPlots/EventTaggingEfficiency_HighMass.pdf}}
% \subfigure[Low mass region]{
% \includegraphics[scale=0.4, angle=0]{figure/FinalPlots/EventTaggingRate_lowmass.pdf}}
% \end{center}
% \caption{The per-event b -tagging efficiencies after the event selection as a function of the reconstructed invariant mass, mjj, 
% for simulated event samples with (a) seven different $b^*$ and $Z'$ resonance masses at high-mass region and (b) four different $Z'$ resonance masses at low-mass region.}
% \label{fig:eventtageff}
% \end{figure}

\begin{figure}[!ht]
\begin{center}
\subfigure[High mass region]{
\includegraphics[scale=0.6, angle=0]{figure/FinalPlots/signal_event_efficiency_fin.pdf}}
\subfigure[Low mass region]{
\includegraphics[scale=0.6, angle=0]{figure/FinalPlots/signal_event_efficiency_low_fin.pdf}}
\end{center}
\caption{Signal acceptance times efficiency  for  inclusive 1 $b$-tag and 2 $b$-tag categories as a function of the simulated $b^*$  and the $Z'$ masses. }
\label{fig:signaleventeff}
\end{figure}

\begin{figure}[!ht]
\begin{center}
\subfigure[Inclusive]{
\includegraphics[width=0.45\linewidth, angle=0]{figure/FinalPlots/flaverComp_mass_fin.pdf}}
\subfigure[Inclusive one $b$-tag]{
\includegraphics[width=0.45\linewidth, angle=0]{figure/FinalPlots/flaverComp_mass_b_fin.pdf}}
\subfigure[Two $b$-tag]{
\includegraphics[width=0.45\linewidth, angle=0]{figure/FinalPlots/flaverComp_mass_bb_fin.pdf}}
\end{center}
\caption{The flavor composition of the simulated dijet background as a function of dijet mass  (a) before tagging, (b) with inclusive one $b$-tag and  (c) with two $b$-tags. The fraction of the six combinations of the $b$-jet , $c$-jet and light-flavor jet are shown. All offline selections are applied.
}
\label{fig:flavourcomp}
\end{figure}

\begin{figure}[!htb]
\begin{center}
\includegraphics[width=0.6\linewidth, angle=0]{figure/FinalPlots/GenericGaussians_inclub_highmass_3_7_10_15_fold_fin_expected.pdf}\caption{Observed (filled circles) and expected (dotted line)  95\% credibility-level upper limits on $\sigma \times A \times \epsilon \times {\mathcal{B}}(X \to b\bar{b})$, including kinematic acceptance and $b$-tagging efficiencies, for resonances exhibiting a generic Gaussian shape at particle level. The plot shows the limits obtained from the inclusive $b$-jet selection. The limits corresponding to Gaussian-shaped resonances with width of $\Gamma_{X}/m_{X} = 3\%$ (red inverted triangles), 7\% (green triangles), 10\% (blue square) and 15\% (purple dots) are shown.}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.6\linewidth, angle=0]{figure/FinalPlots/GenericGaussians_bb_combined_3_7_10_15_fold_finexpected.pdf}\caption{Observed (filled circles) and expected (dotted line)  95\% credibility-level upper limits on $\sigma \times A \times \epsilon \times {\mathcal{B}}(X \to b\bar{b})$, including kinematic acceptance and $b$-tagging efficiencies, for resonances exhibiting a generic Gaussian shape at particle level. The plot shows the limits obtained from the combined low- and high-mass (separated by the vertical dotted line) two $b$-tags selection. The limits corresponding to Gaussian-shaped resonances with width of $\Gamma_{X}/m_{X} = 3\%$ (red inverted triangles), 7\% (green triangles), 10\% (blue square) and 15\% (purple dots) are shown.}
\end{center}
\end{figure}

